SpikeReveal: Unlocking Temporal Sequences from Real Blurry Inputs with Spike Streams

Reconstructing a sequence of sharp images from the blurry input is crucial for enhancing our insights into the captured scene and poses a significant challenge due to the limited temporal features embedded in the image. Spike cameras, sampling at rates up to 40,000 Hz, have proven effective in capturing motion features and beneficial for solving this ill-posed problem. Nonetheless, existing methods fall into the supervised learning paradigm, which suffers from notable performance degradation when applied to real-world scenarios that diverge from the synthetic training data domain. Moreover, the quality of reconstructed images is capped by the generated images based on motion analysis interpolation, which inherently differs from the actual scene, affecting the generalization ability of these methods in real high-speed scenarios. To address these challenges, we propose the first self-supervised framework for the task of spike-guided motion deblurring. Our approach begins with the formulation of a spike-guided deblurring model that explores the theoretical relationships among spike streams, blurry images, and their corresponding sharp sequences. We subsequently develop a self-supervised cascaded framework to alleviate the issues of spike noise and spatial-resolution mismatching encountered in the deblurring model. With knowledge distillation and re-blurring loss, we further design a lightweight deblur network to generate high-quality sequences with brightness and texture consistency with the original input. Quantitative and qualitative experiments conducted on our real-world and synthetic datasets with spikes validate the superior generalization of the proposed framework. Our code, data and trained models will be available at \url{https://github.com/chenkang455/S-SDM}.

==> figs/main/SDM_BSN_SR.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/SDM_BSN_SR.pdf}
    \caption{The schematic diagram presents the SDM model (a), the denoising network (b), and the SR network (c). In these diagrams, ``\MyEmoji{\fire}" symbolizes the network is trained during this stage. Additionally, the black hole in (b) signifies that the information in this area is not accessible to the BSN.}
    \label{fig:SDM_BSN_SR}
        % \vspace{-2em}
\end{figure}


==> figs/main/ablation1.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \begin{subfigure}[b]{0.412\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0cm}, clip]{imgs/Ablation/gopro_aba_110_ablation1/out/Blur_large.png}
        %\vspace{-1.7em}
        \subcaption*{\centering Blurry Input}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_aba_110_ablation1/out/Blur.png}
        %\vspace{-1.7em}
        \subcaption*{\centering Blur}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_aba_110_ablation1/out/BSN_SR.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-3}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_aba_110_ablation1/out/TFP_RESIZE.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-1}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_aba_110_ablation1/out/Deblur.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-4}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_aba_110_ablation1/out/BSN_RESIZE.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-2}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_aba_110_ablation1/out/GT.png}
        %\vspace{-1.7em}
        \subcaption*{\centering GT}
        \end{subfigure}
    \end{subfigure}
    %%% ---------
        \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \begin{subfigure}[b]{0.412\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0cm}, clip]{imgs/Ablation/gopro_car_32_ablation1/out/Blur_large.png}
        %\vspace{-1.7em}
        \subcaption*{\centering Blurry Input}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car_32_ablation1/out/Blur.png}
        %\vspace{-1.7em}
        \subcaption*{\centering Blur}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car_32_ablation1/out/BSN_SR.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-3}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car_32_ablation1/out/TFP_RESIZE.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-1}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car_32_ablation1/out/Deblur.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-4}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car_32_ablation1/out/BSN_RESIZE.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-2}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car_32_ablation1/out/GT.png}
        %\vspace{-1.7em}
        \subcaption*{\centering GT}
        \end{subfigure}
    \end{subfigure}
\\ 
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \begin{subfigure}[b]{0.412\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0cm}, clip]{imgs/Ablation/gopro_person_97_ablation1/out/Blur_large.png}
        %\vspace{-1.7em}
        \subcaption*{\centering Blurry Input}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_person_97_ablation1/out/Blur.png}
        %\vspace{-1.7em}
        \subcaption*{\centering Blur}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_person_97_ablation1/out/BSN_SR.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-3}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_person_97_ablation1/out/TFP_RESIZE.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-1}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_person_97_ablation1/out/Deblur.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-4}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_person_97_ablation1/out/BSN_RESIZE.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-2}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_person_97_ablation1/out/GT.png}
        %\vspace{-1.7em}
        \subcaption*{\centering GT}
        \end{subfigure}
    \end{subfigure}
    %%% ---------
        \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \begin{subfigure}[b]{0.412\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0cm}, clip]{imgs/Ablation/gopro_car2_994_ablation1/out/Blur_large.png}
        %\vspace{-1.7em}
        \subcaption*{\centering Blurry Input}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car2_994_ablation1/out/Blur.png}
        %\vspace{-1.7em}
        \subcaption*{\centering Blur}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car2_994_ablation1/out/BSN_SR.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-3}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car2_994_ablation1/out/TFP_RESIZE.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-1}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car2_994_ablation1/out/Deblur.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-4}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car2_994_ablation1/out/BSN_RESIZE.png}
        %\vspace{-1.7em}
        \subcaption*{\centering I-2}
        %\vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Ablation/gopro_car2_994_ablation1/out/GT.png}
        %\vspace{-1.7em}
        \subcaption*{\centering GT}
        \end{subfigure}
    \end{subfigure}
	\caption{Ablation study for evaluating modules of S-SDM on the GOPRO dataset. Experiments corresponding to the ID can be viewed through \cref{tab:ablation1}.}
	\label{fig:ablation1}
     \vspace{-2em}
\end{figure*}

==> figs/main/ablation2.tex <==
\def\imwidth{0.24}


\def\redpos{(0.55,0.55)} 
\def\greenpos{(-0.8,0)} 

\def\redtoplace{(-0.02,-1.4)}
\def\greentoplace{(1.45,-1.4)}
\def\hh{1.1cm}
\def\ww{1.43cm}
% spy 框的尺寸
\def\ssizz{10}
\def\sswidth{0.245\textwidth}
% 放大倍数
\def\ssmag{3}
\def\scc{(2.12,1.4)}
\begin{figure*}[t]
\footnotesize
	\centering
    % \subfigure{
    	\begin{minipage}[t]{\imwidth\linewidth}
    		\centering
    		% 1-1
			\begin{tikzpicture}[spy using outlines={chamfered rectangle,green,magnification=\ssmag,size= \ssizz,width = \ww,height = \hh},inner sep=0]
				\node {\includegraphics[width=\linewidth]{imgs/Ablation/distillation_real_calib/raw/Blur.png}};
				\spy on \greenpos in node [left] at \greentoplace;
				\spy [red] on \redpos in node [left,red] at \redtoplace;
				\end{tikzpicture}
            Blurry Image\\
            \vspace{0.28em}
            % 2-1
            \begin{tikzpicture}[spy using outlines={chamfered rectangle,green,magnification=\ssmag,size= \ssizz,width = \ww,height = \hh},inner sep=0]
				\node {\includegraphics[width=\linewidth]{imgs/Ablation/distillation_real_calib/raw/NEW_GOPRO_9_reblur50_24_full_100.png}};
				\spy on \greenpos in node [left] at \greentoplace;
				\spy [red] on \redpos in node [left,red] at \redtoplace;
				\end{tikzpicture}
            
            II-4\\
            \vspace{0.5em}

           
    	\end{minipage}%
    % }
    \hspace*{0mm}
    % \subfigure{
    	\begin{minipage}[t]{\imwidth\linewidth}
    		\centering
      % 1-2
    		\begin{tikzpicture}[spy using outlines={chamfered rectangle,green,magnification=\ssmag,size= \ssizz,width = \ww,height = \hh},inner sep=0]
				\node {\includegraphics[width=\linewidth]{imgs/Ablation/distillation_real_calib/raw/NEW_GOPRO_9_reblur10_24_full_nolpips.png}};
				\spy on \greenpos in node [left] at \greentoplace;
				\spy [red] on \redpos in node [left,red] at \redtoplace;
				\end{tikzpicture}
			II-1\\
			\vspace{0.5em}

   % 2-2
			\begin{tikzpicture}[spy using outlines={chamfered rectangle,green,magnification=\ssmag,size= \ssizz,width = \ww,height = \hh},inner sep=0]
				\node {\includegraphics[width=\linewidth]{imgs/Ablation/distillation_real_calib/raw/NEW_GOPRO_9_reblur70_24_full.png}};
				\spy on \greenpos in node [left] at \greentoplace;
				\spy [red] on \redpos in node [left,red] at \redtoplace;
				\end{tikzpicture}
			II-5\\
		    \vspace{0.5em}
			
    	\end{minipage}%
    % }
    \hspace*{0mm}
    % \subfigure{
    	\begin{minipage}[t]{\imwidth\linewidth}
    		\centering
    % 1-3
            \begin{tikzpicture}[spy using outlines={chamfered rectangle,green,magnification=\ssmag,size= \ssizz,width = \ww,height = \hh},inner sep=0]
				\node {\includegraphics[width=\linewidth]{imgs/Ablation/distillation_real_calib/raw/NEW_GOPRO_9_reblur0_24_100.png}};
				\spy on \greenpos in node [left] at \greentoplace;
				\spy [red] on \redpos in node [left,red] at \redtoplace;
				\end{tikzpicture}
			II-2\\
			\vspace{0.5em}
    		
			\begin{tikzpicture}[spy using outlines={chamfered rectangle,green,magnification=\ssmag,size= \ssizz,width = \ww,height = \hh},inner sep=0]
				\node {\includegraphics[width=\linewidth]{imgs/Ablation/distillation_real_calib/raw/NEW_GOPRO_9_reblur100_24_full_100.png}};
				\spy on \greenpos in node [left] at \greentoplace;
				\spy [red] on \redpos in node [left,red] at \redtoplace;
				\end{tikzpicture}
				
			II-6\\
			\vspace{0.5em}
   \end{minipage}
			%(13.32, 0.4847)\vspace{0.5em} E2SRI
			%(12.22, 0.3836)\vspace{0.5em} e2vid
% 3-3
    \hspace*{0mm}
    % \subfigure{
    	\begin{minipage}[t]{\imwidth\linewidth}
    		\centering
    		% 1-4
    		\begin{tikzpicture}[spy using outlines={chamfered rectangle,green,magnification=\ssmag,size= \ssizz,width = \ww,height = \hh},inner sep=0]
				\node {\includegraphics[width=\linewidth]{imgs/Ablation/distillation_real_calib/raw/NEW_GOPRO_9_reblur10_24_full_100.png}};
				\spy on \greenpos in node [left] at \greentoplace;
				\spy [red] on \redpos in node [left,red] at \redtoplace;
				\end{tikzpicture}
			II-3\\
			\vspace{0.5em}
			% 2-4
			\begin{tikzpicture}[spy using outlines={chamfered rectangle,green,magnification=\ssmag,size= \ssizz,width = \ww,height = \hh},inner sep=0]
				\node {\includegraphics[width=\linewidth]{imgs/Ablation/distillation_real_calib/raw/deblur.png}};
				\spy on \greenpos in node [left] at \greentoplace;
				\spy [red] on \redpos in node [left,red] at \redtoplace;
				\end{tikzpicture}
				
			II-7 (retrained II-6)\\
			\vspace{.5em}
			
    	\end{minipage}%
    \hspace*{0mm}
    \centering
	\caption{Ablation study for evaluating the overall effectiveness of our distillation learning framework on the RSB dataset. The details corresponding to the experiment ID can be viewed through the \cref{tab:ablation2}.}
	\label{fig:ablation2}
    \vspace{-2em}
\end{figure*}

==> figs/main/compare1.tex <==
\def\imwidth{0.187}
\def\cimwid{0.125}
\def\rswidth{0.25}
\def\zuoxia{(-1.2,-0.9)}
\def\youshang{(-0.4,-0.45)}
\def\seqwidth{0.80}
\def\ssyy{(-0.8,-0.85)}
\def\ssizz{1.8cm}
\def\sswidth{0.245\textwidth}
\def\ssmag{2.5}
\def\scc{(2.12,1.4)}
\def\smallboxloc{(-0.52,-0.7)} % 绿色小方框位置
\def\largeboxloc{(2.2, 0.75)} % 绿色大方框位置
\begin{figure*}[!h]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \begin{subfigure}[b]{0.412\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0cm}, clip]{imgs/Compare/compare_real_earphone_1/Blur_large.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Blurry Input}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_earphone_1/Blur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Blur}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_earphone_1/BIT.png}
        % \vspace{-1.7em}
        \subcaption*{\centering BiT}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_earphone_1/LEVS.png}
        % \vspace{-1.7em}
        \subcaption*{\centering LEVS}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_earphone_1/SpkeDeblur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Spk-Net}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_earphone_1/Motion-ETR.png}
        % \vspace{-1.7em}
        \subcaption*{\centering M-ETR} 
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_earphone_1/Deblur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Ours}
        \end{subfigure}
    \end{subfigure}
    %%% ---------
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \begin{subfigure}[b]{0.412\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0cm}, clip]{imgs/Compare/compare_real_calibration_56/Blur_large.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Blurry Input}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_calibration_56/Blur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Blur}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_calibration_56/BIT.png}
        % \vspace{-1.7em}
        \subcaption*{\centering BiT}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_calibration_56/LEVS.png}
        % \vspace{-1.7em}
        \subcaption*{\centering LEVS}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_calibration_56/SpkDeblur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Spk-Net}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_calibration_56/Motion-ETR.png}
        % \vspace{-1.7em}
        \subcaption*{\centering M-ETR}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_calibration_56/Deblur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Ours}
        \end{subfigure}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \begin{subfigure}[b]{0.412\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0cm}, clip]{imgs/Compare/compare_real_kid_2/Blur_large.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Blurry Input}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_kid_2/Blur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Blur}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_kid_2/BIT.png}
        % \vspace{-1.7em}
        \subcaption*{\centering BiT}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_kid_2/LEVS.png}
        % \vspace{-1.7em}
        \subcaption*{\centering LEVS}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_kid_2/SpkDeblur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Spk-Net}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_kid_2/Motion-ETR.png}
        % \vspace{-1.7em}
        \subcaption*{\centering M-ETR} 
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_kid_2/Deblur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Ours}
        \end{subfigure}
    \end{subfigure}
    %%% ---------
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \begin{subfigure}[b]{0.412\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0cm}, clip]{imgs/Compare/compare_real_face_28/Blur_large.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Blurry Input}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_face_28/Blur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Blur}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_face_28/BIT.png}
        % \vspace{-1.7em}
        \subcaption*{\centering BiT}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_face_28/LEVS.png}
        % \vspace{-1.7em}
        \subcaption*{\centering LEVS}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_face_28/SpkDeblur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Spk-Net}
        \end{subfigure}
        %% 
        \begin{subfigure}[b]{0.17\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_face_28/Motion-ETR.png}
        % \vspace{-1.7em}
        \subcaption*{\centering M-ETR}
        % \vspace{-0.2em}
        \includegraphics[width=\linewidth, trim={0cm 0 0cm 0}]{imgs/Compare/compare_real_face_28/Deblur.png}
        % \vspace{-1.7em}
        \subcaption*{\centering Ours}
        \end{subfigure}
    \end{subfigure}
\caption{Qualitative comparisons on the real-world RSB dataset, where `M-ETR' refers to Motion-ETR \cite{motion_etr} and `Spk-Net' is the abbreviation of SpkDeblurNet \cite{spike_deblur}.}
	\label{fig:compare_rsb1}
     \vspace{-2em}
\end{figure*}

==> figs/main/compare_seq.tex <==
\begin{figure*}[h]
\footnotesize
	\centering
        \begin{minipage}[t][3.9cm][t]{\rswidth\textwidth}
        \vspace{0pt}
        \centering
              \begin{tikzpicture}[spy using outlines={rectangle,green,magnification=\ssmag,size=\ssizz},inner sep=0]
        				\node {\includegraphics[width=\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/Blur_large.jpg}};
        				% \spy on \smallboxloc in node [left] at \largeboxloc;
        				\end{tikzpicture}
            
            (a) Blur\vspace{0.3em}
            % \vspace{0.8em}
                    % RS frame \vspace{-0.3em}
             \vfill
			\begin{tikzpicture}[spy using outlines={rectangle,green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/SpkeDeblur_large.jpg}};
				% \spy on \smallboxloc in node [left] at \largeboxloc;
				\end{tikzpicture}
            
           (b) Spk-Net \vspace{0.3em}
           \begin{tikzpicture}[spy using outlines={rectangle,green,magnification=\ssmag,size=\ssizz},inner sep=0]
        				\node {\includegraphics[width=\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/deblur_large.jpg}};
        				% \spy on \smallboxloc in node [left] at \largeboxloc;
        				\end{tikzpicture}
            (c) Ours \vspace{0.3em}
    	\end{minipage}% 
% \hspace*{-1mm}
% \hspace*{-5mm}
\begin{minipage}[t]{\seqwidth\textwidth}
            \vspace{0pt}
    		\centering
      % trim={左，下，右，上}
      \begin{tikzpicture}[inner sep=0]
            \node [label={[label distance=0.2cm,text depth=0ex,rotate=90]right: \textcolor{black}{  \scriptsize LEVS}}] at (0,5) {};
            \end{tikzpicture}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/LEVS/008_0.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/LEVS/008_1.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/LEVS/008_2.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/LEVS/008_3.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/LEVS/008_4.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/LEVS/008_5.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/LEVS/008_6.jpg}
   \\
     % \\
   \vspace{0.465em}
            \begin{tikzpicture}[inner sep=0]
            \node [label={[label distance=0.1cm,text depth=0,rotate=90]right: \textcolor{black}{ \scriptsize M-ETR }}] at (0,5) {};
            \end{tikzpicture}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/Motion-ETR/008_0.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/Motion-ETR/008_1.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/Motion-ETR/008_2.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/Motion-ETR/008_3.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/Motion-ETR/008_4.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/Motion-ETR/008_5.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/Motion-ETR/008_6.jpg}
   \\
   \vspace{0.465em}
            \begin{tikzpicture}[inner sep=0]
            \node [label={[label distance=0.3cm,text depth=-1ex,rotate=90]right: \textcolor{black}{ \scriptsize BiT }}] at (0,8.7) {};
            \end{tikzpicture}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/BIT/008_0.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/BIT/008_1.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/BIT/008_2.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/BIT/008_3.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/BIT/008_4.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/BIT/008_5.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/BIT/008_6.jpg}
    \\
   \vspace{0.465em}
            \begin{tikzpicture}[inner sep=0]
            \node [label={[label distance=0.1cm,text depth=-1ex,rotate=90]right: \textcolor{black}{ \scriptsize Spk-Net }}] at (-20,1) {};
            \end{tikzpicture}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/SpkDeblur/008_0.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/SpkDeblur/008_1.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/SpkDeblur/008_2.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/SpkDeblur/008_3.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/SpkDeblur/008_4.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/SpkDeblur/008_5.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/SpkDeblur/008_6.jpg}
   \\
   \vspace{0.465em}
            \begin{tikzpicture}[inner sep=0]
            \node [label={[label distance=0.3cm,text depth=-1ex,rotate=90]right: \textcolor{black}{ \scriptsize Ours }}] at (0,8.7) {};
            \end{tikzpicture}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/deblur/008_0.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/deblur/008_1.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/deblur/008_2.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/deblur/008_3.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/deblur/008_4.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/deblur/008_5.jpg}
			\includegraphics[width=\cimwid\linewidth]{imgs/Compare/compare_seq_middle_calib_8/out/deblur/008_6.jpg}
    \end{minipage}
    \vspace{1em}
	\caption{Qualitative comparison for the sequence reconstruction on the RSB dataset, where `M-ETR' refers to Motion-ETR \cite{motion_etr} and `Spk-Net' denotes SpkDeblurNet \cite{spike_deblur}. }
	\label{fig:compare_sequence}
 \vspace{-2em}
\end{figure*}

==> figs/main/spike_camera.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{imgs/spikecamera.png}
    \caption{The schematic diagram illustrating the generation mechanism of the spike.}
    \label{fig:spikecamera}
    % \vspace{-5em}
\end{figure}


==> tab/main/ablation1.tex <==
\begin{table}[htbp]
\caption{Ablation study for evaluating the performance of each individual module within our framewor.}
\label{tab:ablation1}
\centering
\begin{tabularx}{0.9\textwidth}{
  >{\centering\arraybackslash}X|
  >{\centering\arraybackslash}X
  >{\centering\arraybackslash}X
  >{\centering\arraybackslash}X|
  >{\centering\arraybackslash}X
  >{\centering\arraybackslash}X
  >{\centering\arraybackslash}X
}
\toprule[2pt]
ID & BSN & SR & LDN  & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
I-1 & $\times$ & & & 22.943 & 0.461 & 0.567 \\
I-2 & $\checkmark$ & & & 24.490 & 0.645 & 0.411 \\
I-3 & $\checkmark$ & $\checkmark$ & & 26.144 & 0.708 & 0.349 \\
I-4 & $\checkmark$ & $\checkmark$ &  $\checkmark$ & \textbf{27.928} & \textbf{0.786} & \textbf{0.252} \\
\bottomrule[2pt]
\end{tabularx}
\end{table}



==> tab/main/ablation2.tex <==
\begin{table}[htbp]
\caption{Ablation study for evaluating the overall effectiveness of our distillation learning framework.}
\label{tab:ablation2}
\centering
\begin{tabularx}{0.9\textwidth}{
  >{\centering\arraybackslash}X|
  >{\centering\arraybackslash}X
  >{\centering\arraybackslash}X
  >{\centering\arraybackslash}X|
  >{\centering\arraybackslash}X
  >{\centering\arraybackslash}X
  >{\centering\arraybackslash}X
}
\toprule[2pt]
ID & $\mathcal{L}_{tea}$ & $\mathcal{L}_{reblur}$ & $\lambda$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
II-1  & $\times$       & $\checkmark$     & 10 & 23.102 & 0.441 & 0.552 \\
II-2  & $\checkmark$   & $\times$ & / & 26.713 & 0.723 & 0.266 \\
II-3  & $\checkmark$   & $\checkmark$     & 10 & 27.380 & 0.762 & 0.259 \\
II-4  & $\checkmark$   & $\checkmark$     & 50 & 27.804 & 0.779 & 0.254 \\
II-5  & $\checkmark$   & $\checkmark$     & 70 & 27.825 & 0.780 & 0.255 \\
II-6  & $\checkmark$   & $\checkmark$    & 100 & \textbf{27.928} & \textbf{0.786} & \textbf{0.252} \\
\bottomrule[2pt]
\end{tabularx}
\end{table}
